Disentangleing Content and Fine-grained Prosody Information via Hybrid ASR Bottleneck Features for Voice Conversion

Non-parallel data voice conversion (VC) have achieved considerable breakthroughs recently through introducing bottleneck features (BNFs) extracted by the automatic speech recognition(ASR) model. However, selection of BNFs have a significant impact on VC result. For example, when extracting BNFs from ASR trained with Cross Entropy loss (CE-BNFs) and feeding into neural network to train a VC system, the timbre similarity of converted speech is significantly degraded. If BNFs are extracted from ASR trained using Connectionist Temporal Classification loss (CTC-BNFs), the naturalness of the converted speech may decrease. This phenomenon is caused by the difference of information contained in BNFs. In this paper, we proposed an any-to-one VC method using hybrid bottleneck features extracted from CTC-BNFs and CE-BNFs to complement each other advantages. Gradient reversal layer and instance normalization were used to extract prosody information from CE-BNFs and content information from CTC-BNFs. Auto-regressive decoder and Hifi-GAN vocoder were used to generate high-quality waveform. Experimental results show that our proposed method achieves higher similarity, naturalness, quality than baseline method and reveals the differences between the information contained in CE-BNFs and CTC-BNFs as well as the influence they have on the converted speech.

==> content/1_related_work.tex <==
\section{Related works}
\label{sec:related}


\subsection{Recognition-synthesis based Voice conversion system}

A key problem in voice conversion is information disentanglement, such as disentangling linguistic and speaker information. Qian et al.\cite{qian2020unsupervised} proposed a disentangle method in a self-supervised manner. However, it is difficult to train this kind of model and the quality of converted waveform is limited. Sun et al.\cite{sun2016phonetic} proposed approach generates PPGs by employing an automatic speech recognition (ASR) system to disentangle the linguistic and speaker information. Considering automatic speech recognition system is trained with large corpus and the training target is to map the acoustic features to transcripts, they mentioned that the variation of speaker information will be equalized to a certain extent.

The output of the automatic speech recognition system is then fed into a synthesizer network. Sun et al.\cite{sun2016phonetic} fed the output of ASR system into a deep bidirectional long short memory(BLSTM) model\cite{hochreiter1997long} for generating converted speech. Zhang et al.\cite{zhang2020voice} used Transformer TTS\cite{li2019neural} module with multi-speaker condition to generate converted acoustic feature. In this paper, we proposed a auto-regressive synthesizer with location-sensitive attention\cite{chorowski2015attention} to generate high quality Mel-spectrograms.
A ordinary Recognition-synthesis based VC system structure is shown in Figure \ref{fig:baseline_img}. We trained two system in Figure \ref{fig:baseline_img} with different ASR system as our baselines.






\subsection{Phonetic posteriorgrams and bottleneck feature}

For recognition stage in ASR coustic model, we extract speaker independent PPG or BN features from the prior layers. The frame based posterior probabilities of phonetic classes or BN are treated as content information. In this stage, various of architectures of model are used like DFSMN\cite{zhang2018deep}, TDNN\cite{peddinti2015time} and  Conformer\cite{gulati2020conformer}. 
One of the most important 
factor to influence the information contained in PPGs or BN is the training loss function as well as the format of the training data i.e if time-aligned label are used. For cross entropy loss, time-aligned label is needed while CTC loss don't.

In our experiment, CE based VC system will generate converted waveform with higher naturalness but lower similarity and quality , which means there have an extra information of prosody and speaker information form source speaker in CE bottleneck feature.
Conversely, the generated waveform from CTC based VC system sometimes lack of naturalness due to the prosody information predicted by neural networks may not accurate enough. However, fewer timbre information from source speaker preserved in CTC bottleneck features and lead to higher similarity and quality.  

% A simple hypothesis to this phenomenon can be formulated as follow:
% \begin{equation}
% \small
% \label{eq:hypothesis_1}
% \{{Phn}_{j}\} = ASR(F_{j}) 
% \end{equation}

% \begin{equation}
% \small
% \label{eq:hypothesis_2}
% \{B_{i},..,Phn_{j},..B_{k}\} = ASR(F_{i},..,F_{k})
% \end{equation}

% Where $Phn$ is the ground truth phoneme label, $F$ is the input acoustic feature frame and $B$ is the $<blank>$ token. 

% For CE loss function in Eq.\ref{eq:hypothesis_1}, each acoustic feature frame need to output a correct phoneme label. It is necessary for network to preserve as much as possible information in each frame . 
% For CTC loss function in Eq.\ref{eq:hypothesis_2} the network only need to have one correct label frame in the duration time of current phoneme. When facing an acoustic feature frame which don't have enough information, the network tend to predict $<blank>$ token instead of trying to extract enough information for this frame.

For CE loss function, the network tend to output correct phoneme label for all acoustic features. It is necessary for network to preserve as much as possible information in each frame. So that redundant information like timbre and prosody also preserved in BN.
CTC loss function make the network tend to predict a pike-like probability distributions due to the introduction of $<blank>$ token. when facing an acoustic feature frame which don't have enough information, the network the network tend to predict $<blank>$ token instead of trying to extract enough information for this frame.

More experimental result could be seen in \textbf{section 4.1}. In this paper, we considered the information contained in CTC Bottleneck feature as content information.






%长河： Introduce 和 related work不要写实验
%2.1部分的内容可以放到Intro的第一段。修建修建
%Intro的第一段不要太长

%2.2 实验相关的就放到Exp就可以了

\input{content/baseline_img}







==> table/ablation_.tex <==



\begin{table}[h]

	\caption{
	The MOS with 95\% confidence intervals shows the impact of different modules in network on naturalness, similarity and quality. \textbf{Mel-Prosody encoder} row is the result gained by feeding mel-spectrogram into prosody encoder to extract prosody embedding.
	}
	
	\label{tab:ablation}
	\centering
% 	\resizebox{\textwidth}{}{

% 	\resizebox{\textwidth}{}{
	\begin{tabular}{lccc}
		\toprule
		 &\small{Naturalness} 
		 &\small{Similarity} 
		 &\small{Quality}\\
        \midrule
        
		\small{Proposed} 
		&\textbf{3.65±0.136} 
		&\textbf{3.75±0.136}  
		&\textbf{3.96±0.155} \\ 
		
        \small{w/o IN} 
        &3.16±0.171
        &2.89±0.142 
        &2.90±0.153 \\ 
        
        \small{w/o Prosody predictor} 
        &3.0±0.183
        &3.2±0.159 
        &3.2±0.180 \\
        
        \small{w/o Adv predictor} 
        &3.2±0.156 
        &3.4±0.145 
        &3.6±0.160 \\ 
        
        \small{Mel-Prosody encoder} 
        &2.2±0.186
        &2.3±0.157
        &2.8±0.179\\ 
        
		\bottomrule
	\end{tabular}
\end{table}
